Sensitivity studies on the CKM angle $\gamma$ in $\Lambda_b^0 \to D\Lambda$ decays

The sensitivity of the CKM angle $\gamma$ in $\Lambda_b^0 \to D \Lambda$ decays has been studied using the decay parameter $\alpha$ as an observable in addition to the decay rate asymmetry. Feasibility studies show that adding this observable improves the sensitivity on $\gamma$ by up to 60\% and makes the decays one of the most promising places to measure angle $\gamma$ and to search for $C\!P$ violation in $b$-baryon decays.

==> README <==
* Draft of review for AHEP

The template is with minimal style setting, subject to change when the journal template is available.

According to the meeting on 19/05/2021, the person responsible for each chapter is:

- Zhenwei: Introduction (introduction.tex)
- Yanxi: Heavy hadron production and spectroscopy (production.tex)
- Wenbin: CPV in b (beautyCPV.tex)
- Shanzhen: CPV in c (charmCPV.tex)
- Yuehong: Rare decays (raredecay.tex)
- Yiming: Upgrade and prospects (upgrade.tex)

Please edit the .tex file of the chapter you are assigned.
Put all the figures of that chapter in ./figs/<chapter name>, where <chapter name> is the same as your .tex file.
Use LHCb references from LHCb-xxx.bib, and non-LHCb papers as exported from INSPIRE.
Add non-LHCb entries in main.bib under your name.
Label sections as \label{sec:xxx}, similarly \label{fig:xxx} and \label{tab:xxx} for figures and tables.


